Nonlinear soft mode action for the large-$p$ SYK model

The physics of the SYK model at low temperatures is dominated by a soft mode governed by the Schwarzian action. In arXiv:1604.07818 the linearised action was derived from the soft mode contribution to the four-point function, and physical arguments were presented for its nonlinear completion to the Schwarzian. In this paper, we give two derivations of the full nonlinear effective action in the large $p$ limit, where $p$ is the number of fermions in the interaction terms of the Hamiltonian. The first derivation uses that the collective field action of the large-$p$ SYK model is Liouville theory with a non-conformal boundary condition that we study in conformal perturbation theory. This derivation can be viewed as an explicit version of the renormalisation group argument for the nonlinear soft mode action in arXiv:1711.08467. The second derivation uses an Ansatz for how the soft mode embeds into the microscopic configuration space of the collective fields. We generalise our results for the large-$p$ SYK chain and obtain a "Schwarzian chain" effective action for it. These derivations showcase that the large-$p$ SYK model is a rare system, in which there is sufficient control over the microscopic dynamics, so that an effective description can be derived for it without the need for extra assumptions or matching (in the effective field theory sense).

==> Firstpages.tex <==


% format
\baselineskip=18pt  % a la harvmac
\numberwithin{equation}{section}  % make eq labels (sec.num)
\allowdisplaybreaks  % allow page breaks in displayed eqs


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%        TITLE BEGINS HERE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% ========== title (note version) begins here ==========
%
%\vspace*{-1cm}
%\begin{center}
% {\Large\bf Title of the Document}
%\end{center}
%\vspace*{-.5cm}
%
%% ========== title (note version) ends here ==========

%% ========== title (paper version, a la harvmac) begins here ==========

\thispagestyle{empty}

% Report number if necessary
%\vspace*{-2cm} 
%\begin{flushright}
%{\tt }\\
%\end{flushright}

% title, authors, affiliation
\vspace*{1cm} 
\begin{center}
{\fontsize{20pt}{23pt}\selectfont\textbf{TITLE}\vspace{10mm}}
 
 \renewcommand{\thefootnote}{}
\begin{center}
 \fontsize{14pt}{23pt}\selectfont{}

\end{center}
\vskip .2cm


 \vspace*{.5cm} 
 \fontsize{12pt}{23pt}\selectfont{{$^1$ }}

  
 {\tt {}}

\vspace*{0.8cm}
\end{center}

 \renewcommand{\thefootnote}{\arabic{footnote}}
 
\begin{center} {\bf Abstract } 
\end{center}
Abstract goes here



%%INSERT AN ABSTRACT HERE
\noindent 

%\vspace*{.5cm}

% abstract
%\noindent


\newpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%           TITLE ENDS HERE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\tableofcontents
\printindex

